Exposing Software Engineering Students to Stressful Projects: Does Diversity Matter?

Software development teams have to face stress caused by deadlines, staff turnover, or individual differences in commitment, expertise, and time zones. While students are typically taught the theory of software project management, their exposure to such stress factors is usually limited. However, preparing students for the stress they will have to endure once they work in project teams is important for their own sake, as well as for the sake of team performance in the face of stress. Team performance has been linked to the diversity of software development teams, but little is known about how diversity influences the stress experienced in teams. In order to shed light on this aspect, we provided students with the opportunity to self-experience the basics of project management in self-organizing teams, and studied the impact of six diversity dimensions on team performance, coping with stressors, and positive perceived learning effects. Three controlled experiments at two universities with a total of 65 participants suggest that the social background impacts the perceived stressors the most, while age and work experience have the highest impact on perceived learnings. Most diversity dimensions have a medium correlation with the quality of work, yet no significant relation to the team performance. This lays the foundation to improve students' training for software engineering teamwork based on their diversity-related needs and to create diversity-sensitive awareness among educators, employers and researchers.

==> content/discussion.tex <==
%!TEX root = ../mm-study.tex


\section{Discussion}
\label{sec:Discussion}

- Studenten: 	- Student Voice?


%\subsection{Stressors, Learnings and Diversity}
%\label{sec:Discussion:DiscussionOfResults}

 \textcolor{red}{TODO}

%The most significant differences in perceived stress were found in the diversity dimension \textit{social background}. In contrast, there was no significant difference within this dimension in the learnings. Conclusion?
%
%Age was not a significant factor in stress, but it was very significant in learning.  
%
%An intriguing observation is that the dimension \textit{sex} affected stress more than in learning, however, in general, had little influence. In this aspect, it is noteworthy that the most diverse team of five in run 3.6 and 3.7 actually consisted of four female students~(\Cref{fig:experiment}), who also had a completely different approach than the other teams, e.g. team members standing around the table. %ggf photo?
%We should differentiate here in the future whether the explicit proportion of women in the team has an influence, as has already been shown in previous studies~\cite{catolino2019c, russo2020e}.
%
%Education, ethnicity and work experience are relatively balanced.
%
%The diversity dimensions whom(?) mentioned motivation as a learning or the lack of it as a stressor did not overlap.
%
%Similarly, there was no significant learning effect between groups on the significant difference in task distribution for age and social background, but for ethnicity.
%
%Those with work experience have higher values than non-workers in terms of time available and learning from it.
%
%The local students had significant stress with the distribution of work, but their efficient task distribution was reported as significant learning during the experiment.


\subsection{Takeaways and Recommandations}

educators
students
researchers

reference to corr-tables

- aktualisiererter Experiment-Scheudule mit erweitere Menge (induktiv abgeleitete Menge) an Stressfaktoren —$>$ Handlungsempfehlung für Curric.


\label{sec:Discussion:TakeawaysForTeachers}



==> content/tables/corr-learnings-diversity.tex <==
\begin{table}[tb]
	\centering
	\caption{All statistically significant differences of learnings and dimensions of diversity.}
	\label{tab:corr-learnings-diversity}
	\begin{tabular}{llr}
	\toprule
        Learnings & Diversity & $p$-value \\ 
	\midrule
        More Knowledge & Age & .036 \\ 
        ~ & Sex & .028 \\ 
        ~ & Ethnicity & .033 \\ 
        Fast Working & Education & .004 \\ 
        Commitment & Education & .012 \\ 
	~ & Work XP \textit{($<$0.5y -- $\geq$05.y)} & .016 \\ 
        Working Alone & Age & .028 \\ 
        Efficiency of Small Teams & Age & .037 \\
        	~ & Work XP \textit{($<$0.5y -- $\geq$05.y)} & .006 \\ 
        Impact of more Time & Age & .012 \\ 
        	~ & Work XP \textit{($<$0.5y -- $\geq$05.y)} & .027 \\ 
        Task Distribution & Ethnicity & .036 \\ 
	Quiet Space& Work XP \textit{($<$0.5y -- $\geq$05.y)} & .028 \\ 
	\bottomrule
\end{tabular}
\end{table}

%\textit{($<$0.5y – $>$05.y)}

==> content/tables/corr-learnings.tex <==
\begin{table*}[tb]
	\centering
	\caption{Linear relation between mentioned learnings.}
	\label{tab:corr-learnings}
	\begin{tabular}{llllllll}
	\toprule
        & Good Comm. & Bigger Teams & More Time & Strategy & Documenter & Time Manag. & Routine \\ 
        \midrule
        Fast Working & ~ & 0.223 (p=0.037)  & ~ & ~ & ~ & ~ & ~ \\ 
        Fast Adaption & ~ & -0.169 (p=0.088)  & -0.214 (p=0.043)  & 0.334 (p=0.003)  & ~ & ~ & ~ \\ 
        Commitment & 0.346 (p=0.002) & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        Small Teams & ~ & 0.479 (p=0.000)  & ~ & ~ & ~ & ~ & ~ \\ 
        More Time & ~ & 0.538 (p=0.000)  & ~ & ~ & ~ & ~ & ~ \\ 
        Quiet Space & ~ & ~ & ~ & ~ & 0.345 (p=0.002)  & ~ & ~ \\ 
        Strategy & ~ & ~ & ~ & ~ & 0.241 (p=0.026)  & ~ & -0.205 (p=0.050)  \\ 
        Task Distribution & ~ & 0.217 (p=0.041)  & ~ & ~ & ~ & 0.267 (p=0.015)  & ~ \\ 
        Freedom of Work & ~ & ~ & ~ & -0.205 (p=0.050)  & ~ & ~ & 0.496 (p=0.000) \\ 
        \bottomrule
	\end{tabular}
\end{table*}

==> content/tables/corr-stressors-diversity.tex <==
\begin{table}[tb]
	\centering
	\caption{All statistically significant differences of stressors and dimensions of diversity.}
	\label{tab:corr-stressors-diversity}
	\begin{tabular}{llr}
	\toprule
	Stressor & Diversity & $p$-value \\ 
	\midrule
        Missing Work Appr. & Social BG \textit{(both – none)} & .048 \\ 
        Task Distribution & Age & .028 \\ 
        ~ & Social BG \textit{(one – none)} & .012 \\ 
        ~ & Social BG \textit{(both – none)}  & .042 \\ 
        Time Management & Sex & .027 \\ 
        Staff Turnover & Social BG \textit{(both – none)} & .036 \\ 
        Ext. Disturbances & Work \textit{($<$0.5y – $\geq$05.y)} & .038 \\  %\textit{($<$1m – $>$2y)} & .030
        Time & Ethnicity & .030 \\ 
        ~ & Work XP \textit{($<$0.5y – $\geq$05.y)} & .042 \\ 
        Boring Task & Sex & .002 \\ 
        ~ & Ethnicity & .016 \\ 
        ~ & Education & .016 \\ 
        ~ & Social BG \textit{(both – none)} & .021 \\ 
        ~ & Work XP \textit{($<$0.5y – $\geq$05.y)} & .006\\ %        ~ & Work XP \textit{($<$1m – $>$2y)} & .046 \\ 
        Lack of Motivation & Sex & .033 \\ 
        ~ & Social BG \textit{(both - none)} & .048 \\ 
        \bottomrule
    \end{tabular}
\end{table}

==> content/tables/corr-stressors-learnings.tex <==
\begin{table*}[tb]
    \centering
    \tiny
    \label{corr-stressors-learnings}
    \caption{Corrleation of stressors and learnings.}
    \begin{tabular}{llllllllllllllll}
    \toprule
        Stressors/Learnings & More Know. & Routine & Fast Work. & Good Comm. & Commitment  & No Prob. & 1er Team & Bigger Teams &  Small Teams & More Time & Strategy & Doc. & Task Distr. & Time Manag. & Freedom \\ 
        \midrule
        Comm. Complexity & ~ & ~ & ~ & 0.378 (p=0.000) & ~ & ~ & ~ & -0.204 (p=0.051) & ~ & -0.257 (p=0.019) & ~ & ~ & ~ & ~ & ~ \\ 
        Task Complexity & -0.230 (p=0.032) & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & 0.298 (p=0.008) & ~ & ~ & ~ & ~ & ~ \\ 
        Large Team & ~ & ~ & ~ & 0.401 (p=0.000) & ~ & ~ & ~ & ~ & 0.438 (p=0.000) & ~ & ~ & ~ & -0.218 (p=0.040) & ~ & ~ \\ 
        Small Team & ~ & ~ & ~ & ~ & ~ & ~ & 0.273 (p=0.013) & 0.343 (p=0.002) & 0.347 (p=0.002) & 0.262 (p=0.017) & ~ & ~ & ~ & ~ & ~ \\ 
        Missing Strategy & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & 0.296 (p=0.008) & ~ & ~ & ~ \\ 
        Time Management & 0.417 (p=0.000) & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & 0.220 (p=0.039) & ~ \\ 
        Misleading Strategy & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & 0.295 (p=0.008) & 0.316 (p=0.0052) & ~ & ~ & ~ \\ 
        No Common Appr. & ~ & ~ & ~ & ~ & ~ & -0.209 (p=0.047) & ~ & ~ & 0.218 (p=0.040) & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        Noise Level & ~ & ~ & ~ & ~ & ~ & ~ & 0.810 (p=0.000) & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        Loss of Key Pers. & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & 0.230 (p=0.032) & ~ & 0.301 (p=0.007) \\ 
        Staff Turnover & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & 0.206 (p=0.049) & ~ & ~ & ~ & 0.276 (p=0.013) & ~ \\ 
        Disturbances & ~ & ~ & ~ & 0.217 (p=0.040) & ~ & ~ & 0.216 (p=0.042) & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        Time & ~ & -0.209 (p=0.047) & 0.350 (p=0.002) & ~ & ~ & ~ & ~ & 0.365 (p=0.001) & ~ & 0.310 (p=0.006) & ~ & ~ & ~ & ~ & ~ \\ 
        Boring Task & ~ & ~ & ~ & ~ & 0.359 (p=0.001) & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        Lack of Commit. & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & 0.259 (p=0.018) \\ 
        \bottomrule
    \end{tabular}
\end{table*}


==> content/tables/corr-stressors.tex <==
\begin{table*}[tb]
    \centering
    \tiny
    \caption{Linear relation between the stressors.}
    \label{tab:corr-stressors}
    \begin{tabular}{llllllllll}
    \toprule
        Stressors & Comm. Compl. & nicht reagiert-stoerer & Large Team & Miss. Strategy & Task Distr. & Noise Level & Staff Turnover & Time & Boring Task \\ 
        \midrule
        Comm. Compl. & ~ & 0.386 (p=0.000) & 0.284 (p=0.010) & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        Task Complexity & -0.231 (p=0.032) & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        nicht reag.-stoerer & 0.386 (p=0.000) & ~ & 0.210 (p=0.046) & 0.231 (p=0.032) & ~ & ~ & ~ & ~ & ~ \\ 
        Large Team & 0.284 (p=0.010) & 0.210 (p=0.046) & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        Small Team & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        Missing Strategy & ~ & 0.231 (p=0.032) & ~ & ~ & ~ & ~ & -0.213 (p=0.044) & -0.216 (p=0.042) & ~ \\ 
        Task Distribution & ~ & ~ & ~ & ~ & ~ & 0.251 (p=0.021) & ~ & ~ & ~ \\ 
        Time Management & ~ & ~ & ~ & ~ & ~ & ~ & ~ & -0.221 (p=0.038) & ~ \\ 
        No Common Appr. & 0.246 (p=0.024) & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ 
        Noise Level & ~ & ~ & ~ & ~ & 0.251 (p=0.021) & ~ & ~ & ~ & ~ \\ 
        Staff Turnover & ~ & ~ & ~ & -0.213 (p=0.044) & ~ & ~ & ~ & ~ & ~ \\ 
        Disturbances & ~ & ~ & ~ & ~ & ~ & 0.328 (p=0.003) & 0.206 (p=0.050) & ~ & ~ \\ 
        Time & ~ & ~ & ~ & -0.216 (p=0.042) & ~ & ~ & ~ & ~ & ~ \\ 
        Overloading & ~ & ~ & ~ & ~ & ~ & ~ & 0.419 (p=0.000) & ~ & ~ \\ 
        Bottleneck & ~ & ~ & ~ & 0.231 (p=0.031) & 0.500 (p=0.000) & ~ & ~ & ~ & ~ \\ 
        Boring Task & ~ & ~ & ~ & ~ & ~ & ~ & ~ & 0.215 (p=0.042) & ~ \\ 
        Lack of Commitment & ~ & ~ & ~ & ~ & ~ & ~ & ~ & 0.217 (p=0.041) & 0.419 (p=0.000) \\ 
        \bottomrule
    \end{tabular}
\end{table*}

==> content/tables/demos.tex <==
\begin{table*}[t]
\centering
\caption{Diversity dimensions represented by the self-reported demographics of the students from all experiments (N=65).}
\label{tab:demos}
\begin{tabular}{l|rr|rrr|rr|rr|rrr|rrrrr}
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{Age} & \multicolumn{3}{c}{Sex} & \multicolumn{2}{c}{Ethnicity} & \multicolumn{2}{c}{Edu. BG} & \multicolumn{3}{c}{Social BG} & \multicolumn{5}{c}{Working XP $\vert$ Prog. XP} \\ 
 & $<21$ & $\geq21$ & f & m & d & local & oth. & high & oth. & both p.& one p. & none & $>2$ yr. & 1-2 yr. & 6 m.-1 yr. & 1-6 m. & $<1$ m. \\
 \midrule
HHZ & 14 & 9 & 6 & 15 & 2 & 20 & 3 & 21 & 2 & 5 & 2 & 16 & 4  $\vert$ 1 & 3 $\vert$ 3 & 5 $\vert$ 2 & 6 $\vert$ 13 & 5 $\vert$ 4 \\
UP1 & 7 & 12 & 7 & 12 & 0 & 18 & 1 & 17 & 2 & 10 & 4 & 5 & 4 $\vert$ 4 & 4 $\vert$ 4 & 2 $\vert$ 4 & 2 $\vert$ 5 & 6 $\vert$ 2 \\
UP2 & 14 & 9 & 4 & 19 & 0 & 18 & 5 & 21 & 2 & 7 & 8 & 8 & 3 $\vert$ 8  & 0 $\vert$ 6 & 4 $\vert$ 2 & 7 $\vert$ 3 & 9 $\vert$ 3 \\ 
$ \sum $ & 35 & 30 & 17 & 46 & 2 & 56 & 9 & 59 & 6 & 22 & 14 & 29 & 11 $\vert$ 13 & 7 $\vert$ 13 & 11 $\vert$ 8 & 15 $\vert$ 21 & 20 $\vert$ 9 \\
\bottomrule
\end{tabular}
\end{table*}

==> content/tables/diverseTeamsExp.tex <==
\begin{table}[tb]
    \centering
    \tiny
    \caption{The absolute values of all teams' mentioned categories for the third sub-experiment (run 3.6 and 3.7). The teams HHZ-D, UP1-C, UP2-D are the control groups. Overloading und noise is not mentioned.}
	\label{tab:diverseTeamsExp}
    \begin{tabular}{lCCCCCCCCCCCr}
    \toprule    
        Category & \multicolumn{1}{c}{HHZ-D} &  \multicolumn{1}{c}{HHZ-C} &  \multicolumn{1}{c}{HHZ-B} &  \multicolumn{1}{c}{HHZ-A}&  \multicolumn{1}{c}{UP2-D} &  \multicolumn{1}{c}{UP2-C} &  \multicolumn{1}{c}{UP2-B} & \multicolumn{1}{c}{UP2-A} &\multicolumn{1}{c}{UP1-C} & \multicolumn{1}{c}{UP1-B} & \multicolumn{1}{c}{UP1-A} & $\sum$ \\ 
        \midrule
        More Knowledge & 1 & 1 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 1 & 0 & 7 \\ 
        Establish Routine & 1 & 0 & 1 & 0 & 0 & 1 & 1 & 0 & 0 & 0 & 2 & 6 \\ 
        Fast Working & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 1 & 2 & 0 & 0 & 4 \\ 
        Fast Adaption & 0 & 1 & 1 & 0 & 2 & 1 & 1 & 1 & 0 & 0 & 0 & 7 \\ 
        Good Communication & 0 & 1 & 3 & 0 & 0 & 3 & 2 & 0 & 0 & 0 & 0 & 9 \\ 
        Commitment & 0 & 1 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 4 \\ 
        No Problems & 0 & 1 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 3 \\ 
        Benefits of Bigger Teams & 2 & 0 & 0 & 2 & 0 & 0 & 1 & 1 & 1 & 0 & 0 & 7 \\ 
        Efficiency of Small Teams & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
        Impact of more Time & 3 & 0 & 1 & 3 & 0 & 0 & 2 & 2 & 0 & 0 & 2 & 13 \\ 
        Benefit of Quiet Space & 2 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 3 \\ 
        Strategy & 1 & 3 & 1 & 1 & 4 & 2 & 2 & 3 & 2 & 3 & 1 & 23 \\ 
        Documenter & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 1 & 0 & 0 & 3 \\ 
        Task Distribution & 2 & 1 & 0 & 3 & 2 & 2 & 0 & 2 & 1 & 1 & 0 & 14 \\ 
        Time Management & 0 & 3 & 1 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 5 \\ 
        Communication Complexity & 0 & 1 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 4 \\ 
        Task Complexity & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 2 \\ 
        Large Team & 0 & 0 & 0 & 1 & 1 & 0 & 1 & 2 & 1 & 0 & 0 & 6 \\ 
        Small Team & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 1 \\ 
        Missing Strategy & 0 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 1 & 2 & 5 \\ 
        Task Distribution & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 1 & 0 & 2 \\ 
        Time Management & 0 & 1 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 3 \\ 
        Misleading Strategy & 0 & 2 & 0 & 0 & 2 & 1 & 1 & 0 & 0 & 0 & 0 & 6 \\ 
        No Common Approach & 0 & 0 & 0 & 1 & 1 & 0 & 0 & 0 & 1 & 1 & 1 & 5 \\ 
        Loss of Key Personnel & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 0 & 1 & 3 \\ 
        Staff Turnover & 0 & 3 & 1 & 1 & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 7 \\ 
        Disturbances & 0 & 3 & 0 & 3 & 0 & 5 & 2 & 2 & 1 & 4 & 4 & 24 \\ 
        Time & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 1 \\ 
        Bottleneck (Resources) & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 1 & 3 \\ 
        Boring Task & 1 & 0 & 2 & 0 & 0 & 0 & 0 & 1 & 2 & 1 & 1 & 8 \\ 
        Lack of Commitment & 1 & 0 & 2 & 0 & 1 & 0 & 0 & 0 & 2 & 2 & 1 & 9 \\ 
        $\sum$ & 15 & 22 & 17 & 19 & 20 & 16 & 16 & 19 & 20 & 16 & 17 & 197 \\ 
        \bottomrule
    \end{tabular}
\end{table}

==> content/tables/diversityTeams.tex <==
\begin{table}[tb]
\centering
\caption{Diversity score of each diversity dimension per team.}
\label{tab:diversityTeams}
\begin{tabular}{lllllll}
\toprule
 & Age & Sex & Ethnics & Education & Social BG & Work \\ \midrule
Team1 &  &  &  &  &  &  \\
Team2 &  &  &  &  &  &  \\
Team3 &  &  &  &  &  &  \\
Team4 &  &  &  &  &  &  \\
Team5 &  &  &  &  &  &  \\
Team6 &  &  &  &  &  &  \\
Team7 &  &  &  &  &  &  \\
Team8 &  &  &  &  &  &  \\
Team9 &  &  &  &  &  &  \\
Team10 &  &  &  &  &  &  \\
Team11 &  &  &  &  &  &  \\
Team12 &  &  &  &  &  &  \\
Team13 &  &  &  &  &  &  \\
Team14 &  &  &  &  &  &  \\ \bottomrule
\end{tabular}
\end{table}



==> content/tables/questionnaire.tex <==
\begin{table}[t]
\centering
\caption{Questionnaire for the students' demographics (scale: SC=single-choise, FT= free text, N=number)}
\label{tab:questionnaire}
\begin{tabular}{lll}
\toprule
ID & Question & Scale \\ \midrule
DE1 & Please enter your Semester. & N \\
DE2 & Please enter your  Study Program. & FT \\
DE3 & What is your age? & N \\
DE4 & What is your sex? & SC \\
DE5 & Please identify your ethnicity. & SC \\
DE6 & Do you have any disabilities? & SC \\
DE7 & What is your educational background? & SC \\
DE8 & What is your social background? & SC \\
DE9 & How much professional work experience do you have? & SC \\ %(incl. working as a student etc.)
DE10 & How experienced are you in programming? & SC \\ \bottomrule
\end{tabular}
\end{table}
